Greetings from a Triparental Planet

In this work of speculative science, scientists from a distant star system explain the emergence and consequences of triparentalism, when three individuals are required for sexual reproduction, which is the standard form of mating on their home world. The report details the evolution of their reproductive system--that is, the conditions under which triparentalism and three self-avoiding mating types emerged as advantageous strategies for sexual reproduction. It also provides an overview of the biological consequences of triparental reproduction with three mating types, including the genetic mechanisms of triparental reproduction, asymmetries between the three mating types, and infection dynamics arising from their different mode of sexual reproduction. The report finishes by discussing how central aspects of their society, such as short-lasting unions among individuals and the rise of a monoculture, might have arisen as a result of their triparental system.

==> Chapters/BackMatterTemplate.tex <==
% Template for BACK MATTER. 

% In general, we will probably just slot in some PDFs of the editorial board, About the SFI Press, catalog, etc. 

% Use the same \includepdf command that we did for the front matter, linking to a PDF in the directory. 

% e.g., 
% \includepdf{EdBoard.pdf}
% \includepdf{AboutSFIPress.pdf}

==> Chapters/Commands.tex <==
% This document lays out all the COMMANDS that you'd need to know in order to use this template. Don't pay attention to the line-by-line formatting--it's ugly! 

\pagestyle{empty}

%\newgeometry{left=2.5in, right=1in, marginparwidth=120pt, marginparsep=25pt}
%\reversemarginpar
\nonzeroparskip
\setlength{\parindent}{0pt}

\begin{small}

\chapter{How to Use This Guide}

This guide has two functions: (1) to describe the commands you will need in order to use the \texttt{sfimemoir} package, and (2) to provide templates for various parts of a book made with the \texttt{sfimemoir} package. The directory is broken down as follows: 
\begin{itemize}
    \item \texttt{Commands.tex} is the document you are currently reading. This document is essentially the documentation for the package. It includes command definitions, a guide on setting up a chapter, and some basic troubleshooting tips. This should \emph{not} be included in a final book (obviously). The font size is also smaller to accommodate printing.
    \item \texttt{MemoirTemplate.tex} is a template for the ``entire book" document, which calls the chapters one by one using the \texttt{\textbackslash input} command. In InDesign, this is equivalent to the .indb file; in ebooks, this is equivalent to the <spine> element. This document will also include metadata such as the title, editor(s), title glyphs, etc.  
    \item \texttt{FrontMatterTemplate.tex} is a template for a book's front matter. It is pre-loaded with PDFs of the first few pages of a book and provides a line-by-line guide on filling out the front matter for an individual book. 
    \item \texttt{ChapterTemplate.tex} is a template for a given chapter, to be duplicated as needed. 
    \item \texttt{IntroductionTemplate.tex} is a template for a book's introduction, which differs from a chapter in a few key ways (chiefly the chapter heading). This template can also be modified to serve as a base for other non-chapter sections, such as prefaces, appendices, etc. (More on this later.)
    \item \texttt{BackMatterTemplate.tex} is---you guessed it---a template for a book's back matter. However, it's currently blank. This is because back matter will almost definitely be made up of PDFs imported using the \texttt{\textbackslash includepdf} command. 
    \item The \texttt{Graphics} directory, which is pre-populated with some images that will be used in every book. These are called from \texttt{FrontMatterTemplate.tex} and don't need to be touched. 
    \item The \texttt{Bibliographies} directory, which contains a sample bibliography, \texttt{BibTemplate.bib}. 
    \item The two non-\LaTeX\ fonts used by the Press, namely Cochin LT Pro and Glyphabet Plus, both included as \texttt{.otf} files. As much as we might want to put these into a subfolder, the document won't compile unless they're right out there in the main directory. Ah, \LaTeX\ . 
    \item And finally, the One Style to Rule Them All: The package \texttt{sfimemoir}, which will control the design of our book as well as some other structural components. 
\end{itemize}

\chapter{New \& Redefined Commands for the \texttt{sfimemoir} Package}

For the most part, this package adheres to the general \texttt{memoir} class. However, for clarity here is a breakdown of some of the new commands: 

\section{Fonts}

New commands to control fonts and to import the non-\LaTeX\ fonts Glyphabet Plus and Cochin LT Pro. \emph{Note}: Custom font commands such as \texttt{\textbackslash glyphabet\{\textsf{< text >}\}} must be protected on \emph{both} sides with curly brackets, as otherwise they will ``bleed" into all text following. 

\begin{quotation}
\noindent \emph{Example of best practice}: \\ \texttt{Normal text \hl{\{}\textbackslash cochin\{\textsf{< text in Cochin >}\}\hl{\}} normal text.} \\
Normal text {\cochin{text in Cochin}} normal text.
\end{quotation}

Custom font commands are as follows:

\begin{hangparas}{0.6in}{1}

\texttt{\textbackslash normalfont} \\ EB Garamond, Numbers = Oldstyle, LetterSpace = 5

\texttt{\textbackslash textsf} \\ Sans-serif font set to CM Bright. 

\texttt{\textbackslash cmbright} \\ {\cmbright{Will produce text in CM Bright.}}

\texttt{\textbackslash kurier} \\ {\kurier{Will produce text in Kurier Regular.}}

\texttt{\textbackslash kurierchap} \\ {\kurierchap{CHAPTER HEADINGS.}} In the actual chapter headings, these are made all-caps by our style sheet. If you need to use them elsewhere for some reason, must manually make all-caps using \texttt{\textbackslash MakeUppercase}.  

\texttt{\textbackslash kurierbold} \\ {\kurierbold{Will produce text in Kurier Bold.}} 

\texttt{\textbackslash kurierext} \\ Will produce an {\kurierextcaps{extended version}} of Kurier, for quotation lead-ins, etc. 

\texttt{\textbackslash cochin} \\ Will produce text in {\cochin{Cochin LT Pro Italic.}} 

\texttt{\textbackslash glyphabet} \\ Will produce text in the {\glyphabet{GLYPHABET}} (Glyphabet). 

\end{hangparas}

\section{The Title Page}

\begin{tabular}{ l l }
  \texttt{\textbackslash titleglyphs} & \tab Glyphs (all-caps) to be included on the title page \\
   \texttt{\textbackslash title} & \tab Book title \\
   \texttt{\textbackslash subtitle} & \tab Book subtitle \\
   \texttt{\textbackslash author} & \tab = Editor(s) \\
   \texttt{\textbackslash editorslabel} & \tab Either ``editors" or ``editor"; \\
   & \tab for single-author volumes, leave blank \\
   \texttt{\textbackslash date} & \tab Leave blank! \\
\end{tabular}

\section{Other Miscellaneous Useful Commands, New \& Otherwise}

For an extremely helpful list of \LaTeX\ commands, see: \\
http://www.emerson.emory.edu/services/latex/latex\_toc.html

\vspace{0.5cm}

\begin{tabular}{ l l }
 {\kurierbold{Pages}} & \\
  \texttt{\textbackslash cleardoublepage} & \tab Skips to next odd (recto) page. \\
  \texttt{\textbackslash newpage} & \tab Inserts page break. \\
  \texttt{\textbackslash includepdf\{\textsf{< Filename >}.pdf\}} & \tab Inserts a full-page PDF. (But \\
  & \tab make sure PDF is perfectly sized!) \\
  & \\
  {\kurierbold{Spacing}} & \\
  \texttt{\textbackslash vspace\{\textsf{< length >}\}} & \tab Inserts vertical space of \textsf{< length >} \\
  \texttt{\textbackslash hspace\{\textsf{< length >}\}} & \tab Inserts vertical space of \textsf{< length >} \\
  & \\
  {\kurierbold{Symbols}} & \\ 
  \texttt{\textbackslash tab} & \tab Inserts a 12 pt tab \\
  \texttt{\textbackslash textbackslash} & \textbackslash\tab(backslash) \\
  \texttt{\textbackslash textcopyright}   & \textcopyright\tab(copyright symbol) \\
   & \\
  {\kurierbold{Formatting}} & \\ 
  \texttt{\textbackslash hl\{\textsf{< text >}\}} & \hl{text}   Highlights in yellow \\
  \texttt{\textbackslash LaTeX\textbackslash} & \tab Inserts the word \LaTeX\ as it is ``meant" \\
  & \tab to be typeset *eye roll* 
\end{tabular}

\chapter{Converting a Chapter}
\small

When converting a chapter originally written using \texttt{article} or something of that ilk, follow these steps. 

\begin{enumerate}
    \item Scrape the preamble of the \texttt{article} for any packages that may not be called already in the \texttt{sfimemoir} package. Commands that originate in these packages won't work. Group all of these ``orphan" packages in the preamble of the book document (\texttt{BookTitle.tex}).
    \item Make sure that the author info (email, affiliation, mailing address) contained in the \texttt{\textbackslash thanks} commands is saved to Airtable. Then delete it. 
    \item Go through the lines of code in the template, filling things in as necessary. 
\end{enumerate}

\begin{hangparas}{0.6in}{1}

\small

\texttt{\textbackslash begin\{refsection\}} \\ At the top of the chapter, begin a new \texttt{refsection}. We need to indicate the beginning of the chapter so that \texttt{printbibliography} will know where to begin when we call it at the end of the chapter. 

\texttt{\textbackslash includepdf\{} \emph{.pdf} \texttt{\}} \\ Drop in the PDF of the frontispiece image. This is \emph{way} easier than trying to work with \texttt{mboxes} in \TeX\ . 

\texttt{\textbackslash pagestyle\{myheadings\}} \\ Declare the \texttt{pagestyle}. This is most important for the first chapter following the Introduction, but you can keep it in the template for all chapters. Remember, \texttt{myheadings} has the page numbers as well as title on verso and ``Chapter No.: Chapter Title" on the recto headings. 

\end{hangparas}

\section{Structure of a Chapter}

\section*{The Chapter Heading}

\small
\begin{hangparas}{0.6in}{1}

\texttt{\textbackslash chapter[\textsf{<toc>}]\{\textsf{<title>}\}} \\ Set the title for the chapter. \\ \textsf{toc} = the chapter title as shown in TOC \\ \textsf{title} = chapter title as shown in the chapter heading

\texttt{\textbackslash chaptermark\{\textsf{<Chapter Running Head>}\}} \\ Set the running header for the chapter. This is separate from the regular title to account for some long chapter titles (or titles with long subtitles) that may need to be truncated for running heads.

\texttt{\textbackslash begin\{chapauthor\}} \\ \textsf{<Author 1, Affiliation 1 \\ and Author 2, Affiliation 2>}\\ \texttt{\textbackslash end\{chapauthor\}} \\ Use the \texttt{chapauthor} environment to indicate the chapter's author(s) and their affiliation(s). 

\texttt{\textbackslash addcontentsline\{\textsf{<toc>}\}\{\textsf{<toc>}\}} \\ Manually add the chapter author name(s) to the TOC so that we can put them there without their affiliation(s). 

\texttt{\textbackslash vskip\textbackslash afterchapskip} \\ This simply adds the normal amount of space after the chapter author(s). 

\end{hangparas}

\section*{The Chapter Text}

\begin{hangparas}{0.6in}{1}

\texttt{\textbackslash noindent} \\ Everything that directly follows a header will automatically get assigned a no-indent style (yay), but since the \texttt{\textbackslash chapauthor} environment is artificial (i.e., we made it ourselves, rather than it being built in to TeX), we need to specify no-indent here. The second paragraph and beyond will be automatically indented. 

\end{hangparas}

Following this, simply cut and paste everything in the body text of the original chapter. Cleanup will follow. 

\section*{Ending the Chapter}
At the end of the chapter, make sure you have the following elements: 

\begin{hangparas}{0.6in}{1}

\texttt{\{\textbackslash glyphabet\{E\}\}} \\
Your end-glyph. Note that the \emph{entire} \texttt{\textbackslash glyphabet} command is surrounded by curly brackets. This is called ``protection" since these font commands can easily bleed into other sections (e.g., the rest of the book would be in the Glyphabet!)

\texttt{\textbackslash vspace\{1in\}} \\ This inserts the appropriate amount of space before you call the bibliography. 

\texttt{\textbackslash printbibliography[heading=bibliographysection,title=\{References\}]} \\ We defined the beginning of a \texttt{refsection} at the top of the chapter, so this will include everything from that definition through this command. 

\texttt{\textbackslash end\{refsection\}} \\ ...but we need to remember to end the \texttt{refsection} as well! 

\end{hangparas}

Now the basic typesetting of your chapter is done, so we can hit on two other main topics: Citations and Floats. 

\section{Citations \& Bibliography}
 
We use the \texttt{biblatex-chicago} package to handle all of our citations. This package reads off of the \texttt{bibresource} documents that we called in the Preamble. It searches for the ``nickname" of the source, then matches it with author name and year. For more info, see the ``Bib\LaTeX\ Cheat Sheet" at http://tug.ctan.org/info/biblatex-cheatsheet/biblatex-cheatsheet.pdf. 

Specifically, this line of code controls our \texttt{biblatex-chicago} settings in \texttt{sfimemoir.sty}: 

\begin{verbatim}
    \RequirePackage[noibid,authordate, natbib,isbn=false, % 
    backend=biber]{biblatex-chicago}
\end{verbatim}

To change from author-date to notes-bibliography style, simply swap in \texttt{notes} for \texttt{authordate} in that line. 

Most authors will already know how to use Bib\TeX\ (in this case, actually \texttt{biber}) but these are the basic commands:

\begin{hangparas}{0.6in}{1}
\texttt{\textbackslash autocite\{
\textsf{<bib nickname>} \}} \\ The main command for \texttt{biblatex}. Inserts author name(s) and year, within parentheses. \\ Example: Citing using \texttt{autocite} \autocite{Livermore2018}. 

\texttt{\textbackslash autocite*\{
\textsf{<bib nickname>} \}}\\ Inserts \emph{only} the year in parentheses \autocite*{Livermore2018}.

\end{hangparas}

Some authors may want to use their own versions of the commands. In general, you'll avoid a lot of problems by insisting they use \texttt{autocite} and \texttt{autocite*}. 

\section{Floats}

Floats are boxes that contain objects such as images (or even text). For the SFI Press, we'll be using 3 main types: \texttt{figure}, \texttt{table}, and \texttt{pullquote}. 

There are two main things to remember about floats: 

\begin{enumerate}
    \item Floats position themselves according to guidelines that you lay out for them. Basically, \TeX\ takes your preferences into account, but will put the float wherever it sees most appropriate. There are a few ways to get around this (or at least to be more emphatic in telling \TeX\ what you ``prefer." 
    \item Floats get numbered automatically depending on what type of float they are. Each time \TeX\ runs, it counts them and then re-numbers them, so that all \texttt{figure}s will be numbered sequentially, all \texttt{table}s, etc. by chapter. We don't want \texttt{pullquote}s to get numbered, so we've had to make a workaround on that (below). 
\end{enumerate}

\section*{Positioning Floats}

There are three commands for positioning floats: \texttt{[b]} = bottom of page,  \texttt{[t]} = top of page, \texttt{[h]} = "here" (exactly where I put this command). Add ! if you want to be really emphatic about this. e.g., \texttt{\textbackslash begin\{figure\}[h!]} means "Put this figure exactly here, OR ELSE!"

\section*{Figures}

To include a figure, use the \texttt{figure} environment (aka \texttt{figure} float, since \texttt{figure} is defined as a floating environment. Don't worry about the details). 
Syntax: 

\begin{hangparas}{0.3in}{1}
\texttt{\textbackslash begin\{figure\}[\textsf{< t, b, h, h! etc >}]} \\ \texttt{\textbackslash includegraphics[width=\textbackslash textwidth]\{\textsf{< Graphics path >}\}} \\ \texttt{\textbackslash caption\{\textsf{The caption. Choose to call either} \textbackslash caption \textsf{or} \textbackslash captionrule \textsf{depending on whether the figure is at the top of the bottom of the page}.} \\ \texttt{\textbackslash label\{\textsf{figlabel}\}}
\end{hangparas}
\texttt{\textbackslash end\{figure\}}

Breakdown of these commands: 

\begin{hangparas}{0.6in}{1}

\texttt{\textbackslash includegraphics[width=\textbackslash textwidth]\{ \textsf{< Graphics path >}\}} \\ This tells \TeX\ to put an image here at the same width as the text. All images should be perfectly sized to fit on the page, but this enforces that a little more. \textsf{< Graphics path >} should refer to the document organization, e.g., \texttt{Graphics/1\_Graphics/1\_Fig1.png}. 

\texttt{\textbackslash caption} \\ This inserts a caption \emph{without} a rule underneath. Use for floats that are tagged \texttt{[b]} or \texttt{[b!]}. 

\texttt{\textbackslash captionrule} \\ As you can imagine, this inserts a caption \emph{with} a rule underneath. Use for floats tagged \texttt{[t]} or \texttt{[t!]}. 

\end{hangparas}

\emph{Note}: For floats that have to be manually positioned using \texttt{[h]} or \texttt{[h!]}, choose a caption command that works with the eventual placement. You may need to return to this as the document compiles to make sure things are still right. 


\begin{hangparas}{0.6in}{1}

\texttt{\textbackslash label} \\ Here you add a label for reference. Most authors will have already defined their own labels for figures, which leads to some inconsistency: one author might refer to \texttt{\textbackslash fig:x} for his first figure, while another may refer to \texttt{\textbackslash polaritychart} for hers. If you can, impose a consistent numbering and reference scheme as you go through. This will save you some headaches! 

\end{hangparas}

\section*{Pull Quotes}

The way it works right now, pull quotes are floats whose captions are the pull quote. Syntax: 

\begin{hangparas}{0.3in}{1}
\texttt{\textbackslash begin\{pullquote\}[h!]} \\ \texttt{\textbackslash pullquotetext\{\textsf{< Pull quote text >}\}} 
\end{hangparas}
\texttt{\textbackslash end\{pullquote\}}

\section*{Tables}

Tables are really ugly and annoying in \LaTeX\ . 

\restoregeometry

\end{small}

\chapter{Finishing the Book}

Checklist: 
\begin{enumerate} 
\item Are there duplicate packages called in the preamble?  
\item Are any floats getting pushed off the page? Are captions in the correct style (\texttt{\textbackslash caption} vs. \texttt{\textbackslash captionrule})? 
\item Is the TOC complete? 
\item Do all chapter headings begin on a recto page? 
\item Are there any obvious overfull hboxes that need to be manually corrected (see next chapter)? 
\item Are all quotation marks facing the right way (see next chapter)? 

\end{enumerate}

\chapter{Troubleshooting}

\begin{small}

{\kurierextcaps{Basic Typesetting Issues}}
\addcontentsline{toc}{section}{Basic Typesetting Issues}

\section*{Issue: Symbols are appearing oddly}

Remember that \TeX\ requires you to escape special characters in almost all cases. This can be an issue for bibliographies in particular, as some Bib\TeX\ programs (e.g., BibDesk) allow non-escaped characters which then don't translate on Overleaf. 

General special character descriptions are available here: \\  https://en.wikibooks.org/wiki/LaTeX/Special\_Characters


\section*{Issue: Quotation marks}
The quotation mark symbol (") signifies only \emph{right-handed} typographer's quotes. So, typing \texttt{"word"} will give you \textbf{"}word." 

\emph{Solution:} Use \texttt{``\cmbright{< quote >}"}. \\ The left-handed typographer's quotes are made up of the grave accent (same key as tilde).

\emph{Caveat}: For sans-serif fonts, this usually doesn't matter, and can actually look \emph{worse} since the font will actually typeset \texttt{``}, e.g., {\kurier{quotes in ``Kurier"}}. So, for those, just use normal quotation marks "" on both sides. Sigh. 

\section*{Issue: Certain names don't alphabetize properly in bibliography}

Bib\LaTeX\ uses spaces in the \texttt{.bib} entry to distinguish last names from first names. For names like ``De Beers," ``von Trapp," etc., \texttt{biblatex-chicago} knows to alphabetize properly. However, there are rare cases where other names will be listed incorrectly in the bibliography. \\
\emph{Example}: Pieter Rein ten Wolde (a Dutch name)---``Pieter" and ``Rein" are the first and middle names, while ``ten Wolde" is the surname. It appears in the bibliography as 

\begin{quote}
Wolde, Pieter Rein ten. ...
\end{quote}

\emph{Solution}: Surround the surname with curly brackets in the \texttt{.bib} entry. e.g., the \texttt{author} entry for a reference by Pieter Rein ten Wolde---where ``ten Wolde" is the full surname and should be alphabetized under ``T"---would read: 

\begin{verbatim}
    author={{ten Wolde}, Pieter Rein and Becker, Nils B. ...} 
\end{verbatim}

And the bibliography entry would read: 
\begin{quote}
    ten Wolde, Peter Rein. ...
\end{quote}

\section*{"Overfull hboxes"}

You'll get an ``overfull hbox" issue all the time---this means that \TeX\ freaked out about justification. Most of the time this is fine, and \TeX\ will figure out how to hyphenate properly. However, in some cases you'll have to manually add hyphens. Checking this is part of the ``Finishing the Book" checklist in this guide. 

\section{Forewords, Prefaces \& Appendices}

This guide doesn't include a separate Foreword, Preface, or Appendix template. However, these aren't difficult to generate using the \texttt{IntroductionTemplate} document. 

To generate a document for your \texttt{Preface}, duplicate \texttt{IntroductionTemplate.tex} and modify the heading as follows: 

\begin{verbatim}
\chapter*{\LARGE{\glyphabet{P}}} 
{\centering\kurierchap{PREFACE \\}}
\chaptermark{Preface} 
\vskip\midchapskip 
\begin{chapauthor} 
Preface Author, Preface Author Affiliation
\end{chapauthor}
\addcontentsline{toc}{chapter}{Preface} 
\addcontentsline{toc}{section}{Name of Preface Author} 
\vskip\afterchapskip 

\pagestyle{introheadings}
\end{verbatim}

Hopefully this is self-explanatory, but essentially we just replace everything referring to Introduction with Preface, etc. Note that the \texttt{pagestyle} remains the same, as \texttt{introheadings} simply describes a page with no ``Chapter No.: " in the recto heading. 

For an Appendix, you'd additionally delete the lines describing the author(s), as there aren't generally authors on an Appendix. 



\end{small}
